$M_{W_R}$ dependence of leptogenesis in Minimal Left-Right Symmetric Model with different strengths of Type-II seesaw mass

Left Right Symmetric Model (LRSM) being an extension of the Standard model of particle physics incorporates within itself Type-I and Type-II seesaw mass terms naturally. Both the mass terms can have significant amount of contribution to the resulting light neutrino mass within the model and hence on the different phenomenology associated within. In this paper, we have thoroughly analyzed and discussed the implications of specifying different weightages to the type-I and type-II mass terms and also the study has been carried out for different values of $M_{W_R}$ which is mass of the right-handed gauge boson. This paper also gives a deeper insight into the new physics contributions of Neutrinoless Double Beta Decay $(0\nu\beta\beta)$ and their variations with the net baryon asymmetry arising out of the model. Therefore, the main objective of the present paper rests on investigating the implications of imposing different weightage to the type-I and type-II seesaw terms and different values of $M_{W_R}$ on the new physics contributions of $0\nu\beta\beta$ and net baryon asymmetry arising out as a result of resonant leptogenesis. LRSM in this work has been realized using modular group of level 3, $\Gamma(3)$ which is isomorphic to non-abelian discrete symmetry group $A_4$, the advantage being the non-requirement of flavons within the model and hence maintaining the minimality of the model.

==> cite3.tex <==
@article{Kolb:1979ui,
	author = "Kolb, Edward W. and Wolfram, Stephen",
	title = "{The Development of Baryon Asymmetry in the Early Universe}",
	reportNumber = "Print-79-0911 (CAL TECH), OAP-578, CALT-68-752",
	doi = "10.1016/0370-2693(80)90435-9",
	journal = "Phys. Lett. B",
	volume = "91",
	pages = "217--221",
	year = "1980"
}
@article{Altarelli:2012bn,
	author = "Altarelli, Guido and Feruglio, Ferruccio and Merlo, Luca and Stamou, Emmanuel",
	title = "{Discrete Flavour Groups, $theta_{13}$ and Lepton Flavour Violation}",
	eprint = "1205.4670",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	reportNumber = "CERN-PH-TH-2012-137, RM3-TH-12-7, DFPD-2012-TH-4, TUM-HEP-833-12",
	doi = "10.1007/JHEP08(2012)021",
	journal = "JHEP",
	volume = "08",
	pages = "021",
	year = "2012"
}
@article{Taoso:2007qk,
	author = "Taoso, Marco and Bertone, Gianfranco and Masiero, Antonio",
	title = "{Dark Matter Candidates: A Ten-Point Test}",
	eprint = "0711.4996",
	archivePrefix = "arXiv",
	primaryClass = "astro-ph",
	doi = "10.1088/1475-7516/2008/03/022",
	journal = "JCAP",
	volume = "03",
	pages = "022",
	year = "2008"
}
@article{Turner:1993dra,
	author = "Turner, Michael S.",
	title = "{Dark matter: Theoretical perspectives}",
	eprint = "astro-ph/9302003",
	archivePrefix = "arXiv",
	reportNumber = "FERMILAB-CONF-92-382-A",
	doi = "10.1073/pnas.90.11.4827",
	journal = "Proc. Nat. Acad. Sci.",
	volume = "90",
	pages = "4827",
	year = "1993"
}
@article{Minkowski:1977sc,
	author = "Minkowski, Peter",
	title = "{$\mu \to e\gamma$ at a Rate of One Out of $10^{9}$ Muon Decays?}",
	reportNumber = "Print-77-0182 (BERN)",
	doi = "10.1016/0370-2693(77)90435-X",
	journal = "Phys. Lett. B",
	volume = "67",
	pages = "421--428",
	year = "1977"
}
@article{Schechter:1980gr,
	author = "Schechter, J. and Valle, J. W. F.",
	title = "{Neutrino Masses in SU(2) x U(1) Theories}",
	reportNumber = "SU-4217-167, COO-3533-167",
	doi = "10.1103/PhysRevD.22.2227",
	journal = "Phys. Rev. D",
	volume = "22",
	pages = "2227",
	year = "1980"
}
@article{Mohapatra:1979ia,
	author = "Mohapatra, Rabindra N. and Senjanovic, Goran",
	title = "{Neutrino Mass and Spontaneous Parity Nonconservation}",
	reportNumber = "MDDP-TR-80-060, MDDP-PP-80-105, CCNY-HEP-79-10",
	doi = "10.1103/PhysRevLett.44.912",
	journal = "Phys. Rev. Lett.",
	volume = "44",
	pages = "912",
	year = "1980"
}
@article{Wetterich:1981bx,
	author = "Wetterich, C.",
	title = "{Neutrino Masses and the Scale of B-L Violation}",
	reportNumber = "FREIBURG-THEP-81-2",
	doi = "10.1016/0550-3213(81)90279-0",
	journal = "Nucl. Phys. B",
	volume = "187",
	pages = "343--375",
	year = "1981"
}
@article{Antusch:2004xy,
	author = "Antusch, Stefan and King, Steve F.",
	title = "{Type II Leptogenesis and the neutrino mass scale}",
	eprint = "hep-ph/0405093",
	archivePrefix = "arXiv",
	reportNumber = "SHEP-0415",
	doi = "10.1016/j.physletb.2004.07.009",
	journal = "Phys. Lett. B",
	volume = "597",
	pages = "199--207",
	year = "2004"
}
@article{Foot:1988aq,
	author = "Foot, Robert and Lew, H. and He, X. G. and Joshi, Girish C.",
	title = "{Seesaw Neutrino Masses Induced by a Triplet of Leptons}",
	reportNumber = "UM-P-88/89, OZ-P-88/7",
	doi = "10.1007/BF01415558",
	journal = "Z. Phys. C",
	volume = "44",
	pages = "441",
	year = "1989"
}
@article{Haba:2016lxc,
	author = "Haba, Naoyuki and Ishida, Hiroyuki and Yamaguchi, Yuya",
	title = "{Naturalness and lepton number/flavor violation in inverse seesaw models}",
	eprint = "1608.07447",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	reportNumber = "SU-HET-06-2016",
	doi = "10.1007/JHEP11(2016)003",
	journal = "JHEP",
	volume = "11",
	pages = "003",
	year = "2016"
}
@article{Senjanovic:1978ev,
	author = "Senjanovic, Goran",
	title = "{Spontaneous Breakdown of Parity in a Class of Gauge Theories}",
	reportNumber = "CCNY-HEP-78/20",
	doi = "10.1016/0550-3213(79)90604-7",
	journal = "Nucl. Phys. B",
	volume = "153",
	pages = "334--364",
	year = "1979"
}
@article{Senjanovic:2018xtu,
	author = "Senjanovic, Goran and Tello, Vladimir",
	title = "{Disentangling the seesaw mechanism in the minimal left-right symmetric model}",
	eprint = "1812.03790",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1103/PhysRevD.100.115031",
	journal = "Phys. Rev. D",
	volume = "100",
	number = "11",
	pages = "115031",
	year = "2019"
}
@article{BhupalDev:2018xya,
	author = "Bhupal Dev, P. S. and Mohapatra, Rabindra N. and Rodejohann, Werner and Xu, Xun-Jie",
	title = "{Vacuum structure of the left-right symmetric model}",
	eprint = "1811.06869",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1007/JHEP02(2019)154",
	journal = "JHEP",
	volume = "02",
	pages = "154",
	year = "2019"
}
@inproceedings{Grimus:1993fx,
	author = "Grimus, W.",
	title = "{Introduction to left-right symmetric models}",
	booktitle = "{4th Hellenic School on Elementary Particle Physics}",
	reportNumber = "UWTHPH-1993-10",
	pages = "619--632",
	month = "3",
	year = "1993"
}
@article{Mohapatra:1974gc,
	author = "Mohapatra, R. N. and Pati, Jogesh C.",
	title = "{A Natural Left-Right Symmetry}",
	reportNumber = "CCNY-HEP-74-2",
	doi = "10.1103/PhysRevD.11.2558",
	journal = "Phys. Rev. D",
	volume = "11",
	pages = "2558",
	year = "1975"
}
@article{Pati:1974yy,
	author = "Pati, Jogesh C. and Salam, Abdus",
	title = "{Lepton Number as the Fourth Color}",
	reportNumber = "IC-74-7",
	doi = "10.1103/PhysRevD.10.275",
	journal = "Phys. Rev. D",
	volume = "10",
	pages = "275--289",
	year = "1974",
	note = "[Erratum: Phys.Rev.D 11, 703--703 (1975)]"
}
@article{Senjanovic:1975rk,
	author = "Senjanovic, G. and Mohapatra, Rabindra N.",
	title = "{Exact Left-Right Symmetry and Spontaneous Violation of Parity}",
	reportNumber = "CCNY-HEP-75-5",
	doi = "10.1103/PhysRevD.12.1502",
	journal = "Phys. Rev. D",
	volume = "12",
	pages = "1502",
	year = "1975"
}
@phdthesis{Pernow:2019tuf,
	author = "Pernow, Marcus",
	title = "{Phenomenology of SO(10) Grand Unified Theories}",
	school = "Royal Inst. Tech., Stockholm",
	year = "2019"
}
@article{Vergados:2012xy,
	author = "Vergados, J. D. and Ejiri, H. and Simkovic, F.",
	title = "{Theory of Neutrinoless Double Beta Decay}",
	eprint = "1205.0649",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1088/0034-4885/75/10/106301",
	journal = "Rept. Prog. Phys.",
	volume = "75",
	pages = "106301",
	year = "2012"
}
@article{Cardani:2018lje,
	author = "Cardani, L.",
	title = "{Neutrinoless Double Beta Decay Overview}",
	eprint = "1810.12828",
	archivePrefix = "arXiv",
	primaryClass = "nucl-ex",
	doi = "10.21468/SciPostPhysProc.1.024",
	journal = "SciPost Phys. Proc.",
	volume = "1",
	pages = "024",
	year = "2019"
}
@article{Duka:1999uc,
	author = "Duka, P. and Gluza, J. and Zralek, M.",
	title = "{Quantization and renormalization of the manifest left-right symmetric model of electroweak interactions}",
	eprint = "hep-ph/9910279",
	archivePrefix = "arXiv",
	doi = "10.1006/aphy.1999.5988",
	journal = "Annals Phys.",
	volume = "280",
	pages = "336--408",
	year = "2000"
}
@article{Boruah:2022bvf,
	author = "Boruah, Bichitra Bijay and Das, Mrinal Kumar",
	title = "{Realization of Left-Right Symmetric Model by Discrete Flavor Symmetries}",
	doi = "10.1007/978-981-16-5141-0_30",
	journal = "Springer Proc. Phys.",
	volume = "265",
	pages = "285--291",
	year = "2022"
}
@article{Sahu:2020tqe,
	author = "Sahu, Purushottam and Patra, Sudhanwa and Pritimita, Prativa",
	title = "{$A_4$ realization of left-right symmetric linear seesaw}",
	eprint = "2002.06846",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	month = "2",
	year = "2020"
}
@article{Rodejohann:2015hka,
	author = "Rodejohann, Werner and Xu, Xun-Jie",
	title = "{A left\textendash{}right symmetric flavor symmetry model}",
	eprint = "1509.03265",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1140/epjc/s10052-016-3992-1",
	journal = "Eur. Phys. J. C",
	volume = "76",
	number = "3",
	pages = "138",
	year = "2016"
}
@article{Abbas:2020qzc,
	author = "Abbas, Mohammed",
	title = "{Fermion masses and mixing in modular A4 Symmetry}",
	eprint = "2002.01929",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1103/PhysRevD.103.056016",
	journal = "Phys. Rev. D",
	volume = "103",
	number = "5",
	pages = "056016",
	year = "2021"
}
@article{Asaka:2018hyk,
	author = "Asaka, Takehiko and Yoshida, Takahiro",
	title = "{Resonant leptogenesis at TeV-scale and neutrinoless double beta decay}",
	eprint = "1812.11323",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1007/JHEP09(2019)089",
	journal = "JHEP",
	volume = "09",
	pages = "089",
	year = "2019"
}
@article{Blanchet:2009bu,
	author = "Blanchet, Steve and Chacko, Z. and Granor, Solomon S. and Mohapatra, Rabindra N.",
	title = "{Probing Resonant Leptogenesis at the LHC}",
	eprint = "0904.2174",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	reportNumber = "UMD-PP-09-034",
	doi = "10.1103/PhysRevD.82.076008",
	journal = "Phys. Rev. D",
	volume = "82",
	pages = "076008",
	year = "2010"
}
@article{Flanz:1996fb,
	author = "Flanz, Marion and Paschos, Emmanuel A. and Sarkar, Utpal and Weiss, Jan",
	title = "{Baryogenesis through mixing of heavy Majorana neutrinos}",
	eprint = "hep-ph/9607310",
	archivePrefix = "arXiv",
	doi = "10.1016/S0370-2693(96)01337-8",
	journal = "Phys. Lett. B",
	volume = "389",
	pages = "693--699",
	year = "1996"
}
@article{Dev:2015cxa,
	author = "Dev, P. S. Bhupal",
	editor = "Bhuyan, Bipul",
	title = "{TeV Scale Leptogenesis}",
	eprint = "1506.00837",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	reportNumber = "MAN-HEP-2015-08",
	doi = "10.1007/978-3-319-25619-1_38",
	journal = "Springer Proc. Phys.",
	volume = "174",
	pages = "245--253",
	year = "2016"
}
@article{Borgohain:2017akh,
	author = "Borgohain, Happy and Das, Mrinal Kumar",
	title = "{Lepton number violation, lepton flavor violation, and baryogenesis in left-right symmetric model}",
	eprint = "1709.09542",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1103/PhysRevD.96.075021",
	journal = "Phys. Rev. D",
	volume = "96",
	number = "7",
	pages = "075021",
	year = "2017"
}

@article{Barry:2013xxa,
	author = "Barry, James and Rodejohann, Werner",
	title = "{Lepton number and flavour violation in TeV-scale left-right symmetric theories with large left-right mixing}",
	eprint = "1303.6324",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1007/JHEP09(2013)153",
	journal = "JHEP",
	volume = "09",
	pages = "153",
	year = "2013"
}
@article{Chakrabortty:2012mh,
	author = "Chakrabortty, Joydeep and Devi, H. Zeen and Goswami, Srubabati and Patra, Sudhanwa",
	title = "{Neutrinoless double-$\beta$ decay in TeV scale Left-Right symmetric models}",
	eprint = "1204.2527",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1007/JHEP08(2012)008",
	journal = "JHEP",
	volume = "08",
	pages = "008",
	year = "2012"
}
@article{Boruah:2021ktk,
	author = "Boruah, Bichitra Bijay and Das, Mrinal Kumar",
	title = "{Neutrinoless double-beta decay and lepton flavor violation in discrete flavor symmetric left\textendash{}right symmetric model}",
	eprint = "2111.10341",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1142/S0217751X22500269",
	journal = "Int. J. Mod. Phys. A",
	volume = "37",
	number = "06",
	pages = "2250026",
	year = "2022"
}
@article{Borgohain:2017inp,
	author = "Borgohain, Happy and Das, Mrinal Kumar",
	title = "{Neutrinoless double beta decay and lepton flavour violation in broken $\mu-\tau$ symmetric neutrino mass models}",
	eprint = "1705.00922",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1007/s10773-017-3458-8",
	journal = "Int. J. Theor. Phys.",
	volume = "56",
	number = "9",
	pages = "2911--2934",
	year = "2017"
}
@article{Luo:2008rs,
	author = "Luo, M. J. and Liu, Q. Y.",
	title = "{Small Neutrino Masses From Structural cancellation In Left-Right Symmetric Model}",
	eprint = "0812.3453",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1088/1126-6708/2008/12/061",
	journal = "JHEP",
	volume = "12",
	pages = "061",
	year = "2008"
}
@article{King:2020qaj,
	author = "King, Simon J. D. and King, Stephen F.",
	title = "{Fermion mass hierarchies from modular symmetry}",
	eprint = "2002.00969",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1007/JHEP09(2020)043",
	journal = "JHEP",
	volume = "09",
	pages = "043",
	year = "2020"
}
@article{Novichkov:2019sqv,
	author = "Novichkov, P. P. and Penedo, J. T. and Petcov, S. T. and Titov, A. V.",
	title = "{Generalised CP Symmetry in Modular-Invariant Models of Flavour}",
	eprint = "1905.11970",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	reportNumber = "SISSA 14/2019/FISI, IPMU19-0080, IPPP/19/46, CFTP/19-019",
	doi = "10.1007/JHEP07(2019)165",
	journal = "JHEP",
	volume = "07",
	pages = "165",
	year = "2019"
}
@inbook{Feruglio:2017spp,
	author = "Feruglio, Ferruccio",
	editor = "Levy, Aharon and Forte, Stefano and Ridolfi, Giovanni",
	title = "{Are neutrino masses modular forms?}",
	booktitle = "{From My Vast Repertoire ...}: {Guido Altarelli's Legacy}",
	eprint = "1706.08749",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	reportNumber = "DFPD-2017-TH-09",
	doi = "10.1142/9789813238053_0012",
	pages = "227--266",
	year = "2019"
}
@article{Senjanovic:1978ev,
	author = "Senjanovic, Goran",
	title = "{Spontaneous Breakdown of Parity in a Class of Gauge Theories}",
	reportNumber = "CCNY-HEP-78/20",
	doi = "10.1016/0550-3213(79)90604-7",
	journal = "Nucl. Phys. B",
	volume = "153",
	pages = "334--364",
	year = "1979"
}
@article{Xing:2015fdg,
	author = "Xing, Zhi-zhong and Zhao, Zhen-hua",
	title = "{A review of \ensuremath{\mu}-\ensuremath{\tau} flavor symmetry in neutrino physics}",
	eprint = "1512.04207",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1088/0034-4885/79/7/076201",
	journal = "Rept. Prog. Phys.",
	volume = "79",
	number = "7",
	pages = "076201",
	year = "2016"
}
@article{Blanchet:2008pw,
	author = "Blanchet, Steve and Di Bari, Pasquale",
	title = "{New aspects of leptogenesis bounds}",
	eprint = "0807.0743",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1016/j.nuclphysb.2008.08.026",
	journal = "Nucl. Phys. B",
	volume = "807",
	pages = "155--187",
	year = "2009"
}
@article{Buchmuller:2004tu,
	author = "Buchmuller, W. and Di Bari, P. and Plumacher, M.",
	title = "{Some aspects of thermal leptogenesis}",
	eprint = "hep-ph/0406014",
	archivePrefix = "arXiv",
	reportNumber = "DESY-04-093",
	doi = "10.1088/1367-2630/6/1/105",
	journal = "New J. Phys.",
	volume = "6",
	pages = "105",
	year = "2004"
}
@article{Ding:2013bpa,
	author = "Ding, Gui-Jun and King, Stephen F. and Stuart, Alexander J.",
	title = "{Generalised CP and $A_4$ Family Symmetry}",
	eprint = "1307.4212",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1007/JHEP12(2013)006",
	journal = "JHEP",
	volume = "12",
	pages = "006",
	year = "2013"
}
@article{BhupalDev:2014hro,
	author = "Bhupal Dev, P. S. and Lee, Chang-Hun and Mohapatra, R. N.",
	title = "{Leptogenesis Constraints on the Mass of Right-handed Gauge Bosons}",
	eprint = "1408.2820",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	reportNumber = "MAN-HEP-2014-11, UMD-PP-014-014",
	doi = "10.1103/PhysRevD.90.095012",
	journal = "Phys. Rev. D",
	volume = "90",
	number = "9",
	pages = "095012",
	year = "2014"
}
@article{BhupalDev:2015khe,
	author = "Bhupal Dev, P. S. and Lee, Chang-Hun and Mohapatra, R. N.",
	editor = "Mavromatos, Nick E. and Mitsou, Vasiliki A. and Skliros, Dimitri and Di Domenico, Antonio",
	title = "{TeV Scale Lepton Number Violation and Baryogenesis}",
	eprint = "1503.04970",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	reportNumber = "MAN-HEP-2014-17",
	doi = "10.1088/1742-6596/631/1/012007",
	journal = "J. Phys. Conf. Ser.",
	volume = "631",
	number = "1",
	pages = "012007",
	year = "2015"
}
@article{Kakoti:2023isn,
	author = "Kakoti, Ankita and Boruah, Bichitra Bijay and Das, Mrinal Kumar",
	title = "{Minimal left\textendash{}right symmetric model with A4 modular symmetry}",
	eprint = "2301.13552",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1142/S0217751X23501506",
	journal = "Int. J. Mod. Phys. A",
	volume = "38",
	number = "28",
	pages = "2350150",
	year = "2023"
}





